Intelligent Transaction Scheduling via Conflict Prediction in OLTP DBMS

Current architectures for main-memory online transaction processing (OLTP) database management systems (DBMS) typically use random scheduling to assign transactions to threads. This approach achieves uniform load across threads but it ignores the likelihood of conflicts between transactions. If the DBMS could estimate the potential for transaction conflict and then intelligently schedule transactions to avoid conflicts, then the system could improve its performance. Such estimation of transaction conflict, however, is non-trivial for several reasons. First, conflicts occur under complex conditions that are far removed in time from the scheduling decision. Second, transactions must be represented in a compact and efficient manner to allow for fast conflict detection. Third, given some evidence of potential conflict, the DBMS must schedule transactions in such a way that minimizes this conflict. In this paper, we systematically explore the design decisions for solving these problems. We then empirically measure the performance impact of different representations on standard OLTP benchmarks. Our results show that intelligent scheduling using a history increases throughput by $\sim$40\% on 20-core machine.

==> extra.tex <==
The methodology consists of extracting evidence from an aborted transaction that gives some indication of the cause of the abort.
This evidence is also used to cluster incoming transactions. 
The simplest evidence we consider are the {\em references} to a relation attribute, comparison, and value in the WHERE clause of SELECT and UPDATE statements.
These references almost always contain the input parameters to the transaction.
For example, for the SQL in \cref{fig:sql}
the (literal) references are \verb|stock.s_i_id=2| and \verb|stock.s_w_id=5|.
INSERT statements also have references since they are interpreted as being written in the `attribute=value' format.
As a first step, we compute the probability that a transaction aborts given that it makes a specific reference, based on history of aborts. 
The information required for this computation is maintained in the Model component.

% why not also add the update attribute stock.s_quantity=4?



Note that, for a reference {\em attribute=value}, the expected probability of an transaction aborting with a reference to {\em attribute=value} is the number of transactions that aborted that contained the reference divided by the total number of transactions attempted the contained the reference - the sum of the aborted and committed transactions.


